Quantifying the relationship between student enrollment patterns and student performance

Simplified categorizations have often led to college students being labeled as full-time or part-time students. However, at many universities student enrollment patterns can be much more complicated, as it is not uncommon for students to alternate between full-time and part-time enrollment each semester based on finances, scheduling, or family needs. While prior research has established full-time students maintain better outcomes then their part-time counterparts, limited study has examined the impact of enrollment patterns or strategies on academic outcomes. In this paper, we applying a Hidden Markov Model to identify and cluster students' enrollment strategies into three different categorizes: full-time, part-time, and mixed-enrollment strategies. Based the enrollment strategies we investigate and compare the academic performance outcomes of each group, taking into account differences between first-time-in-college students and transfer students. Analysis of data collected from the University of Central Florida from 2008 to 2017 indicates that first-time-in-college students that apply a mixed enrollment strategy are closer in performance to full-time students, as compared to part-time students. More importantly, during their part-time semesters, mixed-enrollment students significantly outperform part-time students. Similarly, analysis of transfer students shows that a mixed-enrollment strategy is correlated a similar graduation rates as the full-time enrollment strategy, and more than double the graduation rate associated with part-time enrollment. Such a finding suggests that increased engagement through the occasional full-time enrollment leads to better overall outcomes.

==> background.tex <==
%\section{Literature Review}

 %Machine learning and data mining tools have recently gained popularity in predicting students academic performance, mainly due to the large size and dimension of the educational data sets. Educational data mining refers to the application of machine learning, statistic and data mining in the field of education. Research in educational data mining are mostly concerned with predicting student performance, identifying at-risk students and determining factors that affect students' outcome \cite{agnihotri2014building,ayan2008prediction,bridgeman2008predicting,choi2018learning,huang2013predicting}. Marbouti, Diefes-Duxb, and Madhavanb \cite{marbouti2016models} applied different machine learning algorithms such as support vector machine, K-nearest neighbors, and naive Bayes classifier to predict students' course grades. The results show that variables such as mid-term and homework grades and in class quizzes are the most important factors in predicting final grades.

%Fike \cite{fike2008predictors} investigated factors that affects fall-to-spring and fall-to-fall retention for 9200 first-time-students. The results of his study show that parameters such as internet-based courses, financial aid, credits enrolled in the first fall semester, and parents education level have significant impact on student's persistence. Soria and Stebleton \cite{soria2012first} compared retention and academic engagement (combining academic participation and identification) for both first-generation and non-first-generation students. First-generation students are those which are first in their family to pursue a bachelor's degree. The results show that first-generation students are more likely to leave school before graduation.  They also are expected to show less academic engagement compared to the non first generation students.

%Nakajima, Dembo and Mossler \cite{nakajima2012student} studied the impact of demographic, academic, financial, and psychosocial variables on students' retention rate and student persistence in colleges. Results indicate that financial aid, work hours, age, and cumulative GPA are the most important factors influencing student persistence; among which cumulative GPA shows the strongest impact. 








